Attention Tracker: Detecting Prompt Injection Attacks in LLMs

Large Language Models (LLMs) have revolutionized various domains but remain vulnerable to prompt injection attacks, where malicious inputs manipulate the model into ignoring original instructions and executing designated action. In this paper, we investigate the underlying mechanisms of these attacks by analyzing the attention patterns within LLMs. We introduce the concept of the distraction effect, where specific attention heads, termed important heads, shift focus from the original instruction to the injected instruction. Building on this discovery, we propose Attention Tracker, a training-free detection method that tracks attention patterns on instruction to detect prompt injection attacks without the need for additional LLM inference. Our method generalizes effectively across diverse models, datasets, and attack types, showing an AUROC improvement of up to 10.0% over existing methods, and performs well even on small LLMs. We demonstrate the robustness of our approach through extensive evaluations and provide insights into safeguarding LLM-integrated systems from prompt injection vulnerabilities.

==> sections/project_page.tex <==
Project Page: \href{https://huggingface.co/spaces/TrustSafeAI/Attention-Tracker-Prompt-Injection-Detector}{\url{https://huggingface.co/spaces/TrustSafeAI/Attention-Tracker-Prompt-Injection-Detector}}

==> tables/random_sen.tex <==
\begin{table*}[ht]
    \centering
    \caption{List of sentences used for finding important heads}
    \begin{tabular}{cc}
        \hline
        The quick brown fox jumps over the lazy dog. & Better safe than sorry. \\
        \hline
        She sells seashells by the seashore. & Don’t bite the hand that feeds you. \\
        \hline
        A journey of a thousand miles begins with a single step. & Don’t cry over spilled milk. \\
        \hline
        The rain in Spain stays mainly in the plain. & A bird in the hand is worth two in the bush. \\
        \hline
        All that glitters is not gold. & A chain is only as strong as its weakest link. \\
        \hline
        To be or not to be, that is the question. & A fool and his money are soon parted. \\
        \hline
        I think, therefore I am. & A house divided against itself cannot stand. \\
        \hline
        Better late than never. & Absence makes the heart grow fonder. \\
        \hline
        Actions speak louder than words. & All good things must come to an end. \\
        \hline
        An apple a day keeps the doctor away. & All roads lead to Rome. \\
        \hline
        The early bird catches the worm. & Appearances can be deceiving. \\
        \hline
        A picture is worth a thousand words. & As the crow flies. \\
        \hline
        Curiosity killed the cat. & As you sow, so shall you reap. \\
        \hline
        Fortune favors the bold. & Beggars can’t be choosers. \\
        \hline
        A penny saved is a penny earned. & Every cloud has a silver lining. \\
        \hline
        Barking dogs seldom bite. & Failing to plan is planning to fail. \\
        \hline
        Beauty is in the eye of the beholder. & Haste makes waste. \\
        \hline
        Birds of a feather flock together. & Honesty is the best policy. \\
        \hline
        Blood is thicker than water. & If it ain’t broke, don’t fix it. \\
        \hline
        Don’t count your chickens before they hatch. & Laughter is the best medicine. \\
        \hline
        Every cloud has a silver lining. & No pain, no gain. \\
        \hline
        Failing to plan is planning to fail. & Out of sight, out of mind. \\
        \hline
        Haste makes waste. & Rome wasn’t built in a day. \\
        \hline
        Honesty is the best policy. & The pen is mightier than the sword. \\
        \hline
        If it ain’t broke, don’t fix it. & Time flies when you’re having fun. \\
        \hline
        Laughter is the best medicine. & Two heads are better than one. \\
        \hline
        No pain, no gain. & When it rains, it pours. \\
        \hline
        Out of sight, out of mind. & Where there’s smoke, there’s fire. \\
        \hline
        Rome wasn’t built in a day. & You can’t judge a book by its cover. \\
        \hline
        The pen is mightier than the sword. & You reap what you sow. \\
        \hline
        Time flies when you’re having fun. & A bird in the hand is worth two in the bush. \\
        \hline
        Two heads are better than one. & A chain is only as strong as its weakest link. \\
        \hline
        When it rains, it pours. & A fool and his money are soon parted. \\
        \hline
        Where there’s smoke, there’s fire. & A house divided against itself cannot stand. \\
        \hline
        You can’t judge a book by its cover. & Absence makes the heart grow fonder. \\
        \hline
        You reap what you sow. & All good things must come to an end. \\
        \hline
    \end{tabular}
    \label{tab:random_sentences}
\end{table*}
